Learning Discriminative Signed Distance Functions from Multi-scale Level-of-detail Features for 3D Anomaly Detection

Detecting anomalies from 3D point clouds has received increasing attention in the field of computer vision, with some group-based or point-based methods achieving impressive results in recent years. However, learning accurate point-wise representations for 3D anomaly detection faces great challenges due to the large scale and sparsity of point clouds. In this study, a surface-based method is proposed for 3D anomaly detection, which learns a discriminative signed distance function using multi-scale level-of-detail features. We first present a Noisy Points Generation (NPG) module to generate different types of noise, thereby facilitating the learning of discriminative features by exposing abnormal points. Then, we introduce a Multi-scale Level-of-detail Feature (MLF) module to capture multi-scale information from a point cloud, which provides both fine-grained local and coarse-grained global feature information. Finally, we design an Implicit Surface Discrimination (ISD) module that leverages the extracted multi-scale features to learn an implicit surface representation of point clouds, which effectively trains a signed distance function to distinguish between abnormal and normal points. Experimental results demonstrate that the proposed method achieves an average object-level AUROC of 92.1\% and 85.9\% on the Anomaly-ShapeNet and Real3D-AD datasets, outperforming the current best approach by 2.1\% and 3.6\%, respectively. Codes are available at https://anonymous.4open.science/r/DLF-3AD-DA61.

==> Supplementary_Material/Supplementary_Material.tex <==
% \textbf{Learning Discriminative Signed Distance Functions with Decoupled Level-of-detail Features for 3D Anomaly Detection—Supplementary Material}
%\input{Supplementary Material/results_Anomoly_O_AUPR}
\newpage
\begin{table*}[h]
  \centering
% \caption{O-AUROC performance of different methods on Real3D-AD across 40 categories, where best and second-place results are highlighted in red and blue, respectively.}
  \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|cccccccccccccc}
    \toprule
    %\multicolumn{15}{c}{\textbf{O-AUROC}} \\
    %\midrule
    \textbf{Method} & \textbf{ashtray0} & \textbf{bag0} & \textbf{bottle0} & \textbf{bottle1} & \textbf{bottle3} & \textbf{bowl0} & \textbf{bowl1} & \textbf{bowl2} & \textbf{bowl3} & \textbf{bowl4} & \textbf{bowl5} & \textbf{bucket0} & \textbf{bucket1} & \textbf{cap0} \\
    \midrule
\textbf{BTF(Raw) (CVPR23’)} & 0.578 & 0.458 & 0.466 & 0.573 & 0.543 & 0.588 & 0.464 & 0.576 & 0.654 & 0.601 & 0.615 & 0.652 & 0.620 & 0.659 \\
\textbf{BTF(FPFH) (CVPR23’)} & 0.651 & 0.551 & 0.644 & 0.625 & 0.602 & 0.576 & 0.648 & 0.515 & 0.499 & 0.632 & 0.699 & 0.483 & 0.648 & 0.618 \\
\textbf{M3DM (CVPR23’)} & 0.632 & 0.642 & 0.763 & 0.674 & 0.451 & 0.525 & 0.515 & 0.630 & 0.635 & 0.571 & 0.601 & 0.609 & 0.507 & 0.564 \\
\textbf{PatchCore(FPFH) (CVPR22’)} & 0.445 & 0.608 & 0.615 & 0.677 & 0.579 & 0.548 & 0.545 & 0.611 & 0.620 & 0.575 & 0.541 & 0.604 & 0.565 & 0.585  \\
\textbf{PatchCore(PointMAE)  (CVPR22')} & \textcolor{blue}{0.679} & 0.601 & 0.545 & 0.645 & 0.651 & 0.562 & 0.611 & 0.456 & 0.556 & 0.601 & 0.585 & 0.541 & 0.642 & 0.561 \\
\textbf{CPMF (PR24’)} & 0.453 & 0.655 & 0.588 & 0.592 & 0.505 & 0.775 & 0.621 & 0.601 & 0.418 & 0.683 & 0.685 & 0.662 & 0.501 & 0.601  \\
\textbf{Reg3D-AD (NeurIPS23’)} & 0.588 & 0.608 & 0.632 & 0.695 & 0.474 & 0.494 & 0.515 & 0.495 & 0.441 & 0.624 & 0.555 & 0.632 & 0.714 & 0.693  \\
\textbf{IMRNet (CVPR24’)} & 0.612 & 0.665 & 0.558 & 0.702 & 0.648 & 0.481 & 0.504 & 0.681 & 0.614 & 0.630 & 0.652 & 0.578 & 0.732 & 0.711  \\
\textbf{PO3AD (CVPR25')} & \textcolor{red}{0.999} & \textcolor{blue}{0.809} & \textcolor{blue}{0.927} & \textcolor{blue}{0.959} & \textcolor{blue}{0.962} & \textcolor{blue}{0.946} & \textcolor{blue}{0.905} & \textcolor{blue}{0.888} & \textcolor{blue}{0.927} & \textcolor{red}{0.985} & \textcolor{blue}{0.904} & \textcolor{blue}{0.923} & \textcolor{blue}{0.882} & \textcolor{blue}{0.841}\\
\textbf{Ours} & \textcolor{red}{0.999} & \textcolor{red}{0.999} & \textcolor{red}{0.999} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{0.982} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{blue}{0.976} & \textcolor{red}{0.991} & \textcolor{red}{0.981} & \textcolor{red}{0.922} & \textcolor{red}{0.934}\\

% \textbf{Reg2Inv(NIPS25')} & \textcolor{blue}{0.900} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & 0.807 & 0.656 & 0.585 & 0.852 & 0.818 & 0.813 & \textcolor{red}{0.902} & 0.659
% \\

    \midrule
    \multicolumn{1}{c}{} &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \textbf{Method} & \textbf{cap3} & \textbf{cap4} & \textbf{cap5} & \textbf{cup0} & \textbf{cup1} & \textbf{eraser0} & \textbf{headset0} & \textbf{headset1} & \textbf{helmet0} & \textbf{helmet1} & \textbf{helmet2} & \textbf{helmet3} & \textbf{jar0} & \textbf{micro.} \\
    \midrule
\textbf{BTF(Raw) (CVPR23’)} & 0.612 & 0.515 & 0.653 & 0.601 & 0.701 & 0.425 & 0.379 & 0.515 & 0.559 & 0.388 & 0.615 & 0.526 & 0.428 & 0.613  \\
\textbf{BTF(FPFH) (CVPR23’)} & 0.579 & 0.545 & 0.593 & 0.585 & 0.651 & 0.719 & 0.531 & 0.523 & 0.568 & 0.721 & 0.588 & 0.564 & 0.479 & 0.662 \\
\textbf{M3DM (CVPR23’)} & 0.652 & 0.477 & 0.642 & 0.570 & \textcolor{blue}{0.752} & 0.625 & 0.632 & 0.623 & 0.528 & 0.627 & 0.636 & 0.458 & 0.555 & 0.464  \\
\textbf{PatchCore(FPFH) (CVPR22’)} & 0.457 & 0.655 & 0.725 & 0.604 & 0.586 & 0.584 & 0.701 & 0.601 & 0.525 & 0.630 & 0.475 & 0.494 & 0.499 & 0.332 \\
\textbf{PatchCore(PointMAE)  (CVPR22')} & 0.583 & \textcolor{blue}{0.721} & 0.542 & 0.642 & 0.710 & 0.801 & 0.515 & 0.423 & 0.633 & 0.571 & 0.496 & 0.611 & 0.463 & 0.652  \\
\textbf{CPMF (PR24’)} & 0.541 & 0.645 & 0.697 & 0.647 & 0.609 & 0.544 & 0.602 & 0.619 & 0.333 & 0.501 & 0.477 & 0.645 & 0.618 & 0.655  \\
\textbf{Reg3D-AD (NeurIPS23’)} & 0.711 & 0.623 & 0.770 & 0.531 & 0.638 & 0.424 & 0.538 & 0.617 & 0.600 & 0.381 & 0.618 & 0.468 & 0.601 & 0.614 \\
\textbf{IMRNet (CVPR24’)} & 0.702 & 0.658 & 0.502 & 0.455 & 0.627 & 0.599 & 0.701 & 0.656 & 0.697 & 0.615 & 0.602 & 0.575 & 0.760 & 0.552  \\
\textbf{PO3AD (CVPR25')} & \textcolor{red}{0.906} & \textcolor{red}{0.876} & \textcolor{blue}{0.801} & \textcolor{blue}{0.879} & \textcolor{red}{0.870} & \textcolor{blue}{0.995} & \textcolor{blue}{0.765} & \textcolor{blue}{0.914} & \textcolor{blue}{0.864} & \textcolor{blue}{0.961} & \textcolor{red}{0.934} & \textcolor{blue}{0.849} & \textcolor{blue}{0.915} & \textcolor{blue}{0.803}\\
\textbf{Ours} & \textcolor{blue}{0.730} & 0.688 & \textcolor{red}{0.853} & \textcolor{red}{0.999} & 0.523 & \textcolor{red}{0.999} & \textcolor{red}{1.000} & \textcolor{red}{0.999} & \textcolor{red}{0.926} & \textcolor{red}{0.991} & \textcolor{blue}{0.744} & \textcolor{red}{0.970} & \textcolor{red}{0.999} & \textcolor{red}{0.999} \\

% \textbf{Reg2Inv(NIPS25')} & \textcolor{red}{0.863} & 0.681 & \textcolor{blue}{0.902} & 0.733 & \textcolor{red}{0.933} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & 0.843 & \textcolor{blue}{0.817} & \textcolor{blue}{0.986} & \textcolor{red}{0.875} & \textcolor{blue}{0.876} & \textcolor{red}{1.000} & \textcolor{red}{1.000}
% \\
    \midrule
    \multicolumn{1}{c}{} &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \textbf{Method} & \textbf{shelf0} & \textbf{tap0} & \textbf{tap1} & \textbf{vase0} & \textbf{vase1} & \textbf{vase2} & \textbf{vase3} & \textbf{vase4} & \textbf{vase5} & \textbf{vase7} & \textbf{vase8} & \textbf{vase9} & \textbf{Average} \\
    \midrule
\textbf{BTF(Raw) (CVPR23’)} & 0.624 & 0.535 & 0.594 & 0.562 & 0.441 & 0.413 & 0.717 & 0.428 & 0.615 & 0.547 & 0.416 & 0.482 & 0.549    \\
\textbf{BTF(FPFH) (CVPR23’)} & 0.611 & 0.610 & 0.575 & 0.641 & 0.655 & 0.569 & 0.652 & 0.587 & 0.472 & 0.592 & 0.624 & 0.638 & 0.598  \\
\textbf{M3DM (CVPR23’)} & 0.665 & 0.722 & 0.638 & \textcolor{blue}{0.788} & 0.652 & 0.615 & 0.551 & 0.526 & 0.633 & 0.648 & 0.463 & 0.651 & 0.603 \\
\textbf{PatchCore(FPFH) (CVPR22’)} & 0.504 & 0.712 & 0.684 & 0.645 & 0.623 & 0.801 & 0.481 & 0.777 & 0.515 & 0.621 & 0.515 & 0.660 & 0.588   \\
\textbf{PatchCore(PointMAE)  (CVPR22')} & 0.543 & 0.712 & 0.542 & 0.548 & 0.572 & 0.711 & 0.455 & 0.586 & 0.585 & 0.652 & 0.655 & 0.634 & 0.595    \\
\textbf{CPMF (PR24’)} & \textcolor{blue}{0.681} & 0.639 & 0.697 & 0.632 & 0.645 & 0.632 & 0.588 & 0.655 & 0.518 & 0.432 & 0.673 & 0.618 & 0.597  \\
\textbf{Reg3D-AD (NeurIPS23’)} & 0.675 & 0.676 & 0.599 & 0.615 & 0.468 & 0.641 & 0.651 & 0.505 & 0.588 & 0.455 & 0.629 & 0.574 & 0.584   \\
\textbf{IMRNet (CVPR24’)} & 0.625 & 0.401 & \textcolor{blue}{0.796} & 0.573 & 0.725 & 0.655 & 0.708 & 0.528 & 0.654 & 0.601 & 0.639 & 0.462 & 0.621 \\
\textbf{PO3AD (CVPR25')} & 0.680 & \textcolor{blue}{0.856} & 0.709 & 0.753 & \textcolor{blue}{0.789} & \textcolor{blue}{0.963} & \textcolor{blue}{0.902} & \textcolor{blue}{0.824} & \textcolor{blue}{0.879} & \textcolor{blue}{0.971} & \textcolor{blue}{0.833} & \textcolor{blue}{0.904} & \textcolor{blue}{0.881}\\
\textbf{Ours} & \textcolor{red}{0.811} & \textcolor{red}{0.921} & \textcolor{red}{0.951} & \textcolor{red}{0.847} & \textcolor{red}{0.976} & \textcolor{red}{0.999} & \textcolor{red}{0.926} & \textcolor{red}{0.916} & \textcolor{red}{0.999} & \textcolor{red}{0.999} & \textcolor{red}{0.956} & \textcolor{red}{0.934} & \textcolor{red}{0.936}\\
% \textbf{Reg2Inv(NIPS25')} & 0.577 & \textcolor{red}{0.948} & 0.804 & \textcolor{blue}{0.996} & 0.605 & \textcolor{red}{1.000} & \textcolor{blue}{0.845} & 0.818 & \textcolor{red}{1.000} & 0.643 & \textcolor{blue}{0.818} & \textcolor{red}{0.873} & 0.861
% \\
    \bottomrule
    \end{tabular}%
}
    \caption{The O-AUPR ($\uparrow$) performance of different methods on Anomaly-ShapeNet, where the best and second-place results are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.}
  \label{results1}
\end{table*}

\section{More Experiment Results}
To further examine the performance of the proposed method, the object-level AUPR (Area Under the Precision-Recall curve) and pixel-level AUPR (Area Under the Precision-Recall curve) were introduced for evaluation.

\subsection{Results on Anomaly-ShapeNet}
Tables ~\ref{results1} and ~\ref{results2} report the anomaly detection and localization results of different methods on the Anomaly-ShapeNet dataset, respectively. The average O-AUPR of the proposed method reached 0.936, surpassing the second-best method by 5.5\%. To our knowledge, there are no publicly available P-AUPR results for the Anomaly-ShapeNet dataset. Nevertheless, our method achieved an average P-AUPR of 0.537, highlighting its effectiveness in anomaly detection across different data categories.
capability across different categories of data.
\input{Supplementary Material/results_Anomoly_P_AUPR}
\input{Supplementary Material/results_Real3D_O_AUPR}
\input{Supplementary Material/results_Real3D_P_AUPR}

\subsection{Experimental Results on Real3D-AD}
Tables~\ref{results3} and ~\ref{results11} show the performance of different methods on the Real3D-AD dataset. The proposed method yielded an average O-AUPR of 0.824 and an average P-AUPR of 0.326, outperforming the best comparison method by 8.4\% and 18.9\%, respectively. These results further verify the superiority of the proposed method for high-precision point clouds.

\section{More Ablation Studies}
\subsection{Effectiveness of the NPG Module} 
To further verify the effectiveness of the proposed Noisy Points Generation (NPG) module, we replaced it with the method of random noise and Norm-AS proposed in PO3AD ~\cite{PO3AD}. The experimental results on the Real3D-AD dataset are shown in Table $\ref{AnomalyGeneration}$.

 \begin{table}[htbp]
  \centering
  \resizebox{0.95\columnwidth}{!}{
    \begin{tabular}{c|ccc}
    \toprule
    \textbf{Method} & Random noise & Norm-AS & NPG (Ours)\\
    \midrule
    O-AUROC &0.659&0.735 &0.859\\
    P-AUROC & 0.557&0.539 &0.852\\
    \bottomrule
    \end{tabular}%
}
   \caption{Experimental results with different anomaly generation methods. }
  \label{AnomalyGeneration}
\end{table}

The method of random noise generates points that are randomly distributed in point cloud space. As shown in $\ref{AnomalyGeneration}$, the performance of the proposed method with random noise is significantly lower than that with the NPG module. This is because unstructured and irregular random points lack geometric correlation with the point cloud surface and cannot simulate the distributions of realistic anomalies.

Norm-AS is an anomaly synthesis method proposed by PO3AD~\cite{PO3AD}, whose core design concept is to generate local pseudo-anomalies through normal vectors. Although this method can realize the anomaly synthesis function, its performance is still inferior to that of the NPG module. The fundamental reason lies in the fact that our proposed method relies on the global surface modeling technology of point clouds, which requires the construction of a complete noise distribution that not only covers the local near-surface area but also includes the global space. However, the local pseudo-anomalies generated by Norm-AS are difficult to meet this requirement.
% Norm-AS is an anomaly synthesis method used in the point-based method PO3AD ~\cite{PO3AD}. Its core idea lies in generating local pseudo-anomalies by predicting point offsets. Although this method can synthesize anomalies, its performance is still inferior to that of the NPG module. The reason is that our proposed method relies on the global surface modeling of point clouds, and thus requires a comprehensive noise distribution that covers both local near-surface regions and global space—a requirement that the local pseudo-anomalies generated by Norm-AS fail to meet.
%In contrast, our NPG module can simulate diverse anomaly scenarios by integrating near-surface noise points ($P_\text{near}$) and uniform noise points ($P_\text{uni}$). This design enables the module to provide sufficient discriminative information for model training. This result further confirms the rationality and superiority of the NPG module in enhancing the model's ability to learn discriminative features for 3D anomaly detection.

%Random noise points are generated as unstructured random points uniformly distributed in space. The performance of the model using this method is significantly lower than that of the model equipped with the NPG module. This is because unstructured random points lack geometric correlation with the point cloud surface and cannot simulate realistic anomaly distributions.
%Norm-AS is an anomaly synthesis method derived from the point-based method PO3AD. Its core lies in generating local pseudo-anomalies by predicting point offsets, which is applied to 3D anomaly detection tasks. Although this method is related to anomaly synthesis, its performance is still inferior to that of the NPG module. The reason is that our proposed method relies on the global surface modeling of point clouds, and thus requires a comprehensive noise distribution that covers both local near-surface regions and global space—a requirement that the local pseudo-anomalies generated by Norm-AS fail to meet.
%In contrast, our NPG module can simulate diverse anomaly scenarios by integrating near-surface noise points ($P_\text{near}$) and uniform noise points ($P_\text{uni}$). This design enables the module to provide sufficient discriminative information for model training. This result further confirms the rationality and superiority of the NPG module in enhancing the model's ability to learn discriminative features for 3D anomaly detection.

\subsection{Effectiveness of the MLF Module}
To verify the superiority of the proposed Multi-scale Level-of-detail Feature (MLF) module in capturing multi-scale geometric features, we conducted comparative experiments on the Real3D-AD dataset by replacing the MLF module with three alternative feature extraction methods, namely FPFH~\cite{BTF}, MLP~\cite{PO3AD}, and PointMAE~\cite {pointmae}. The results are shown in Table~\ref{Feature1}.

As shown in Table~\ref{Feature1}, the proposed method with the MLF module achieved the highest O-AUROC and P-AUROC among all compared methods.
FPFH relies on local geometric descriptors and lacks the ability to extract global structural information. MLP only performs feature mapping and fails to explore correlations between features at different scales. Although PointMAE can extract robust and generalized features through pre-training and masking strategies, it struggles to balance the capture of global context and local fine-grained features. In contrast, the MLF module can accurately capture both global shape structure and local details simultaneously by extracting multi-scale features, thus achieving superior performance in 3D anomaly detection.
 \begin{table}[htbp]
  \centering
  \resizebox{0.95\columnwidth}{!}{
    \begin{tabular}{c|cccc}
    \toprule
    \textbf{Feature} & FPFH& MLP & PointMAE & MLF (Ours)\\
    \midrule
    O-AUROC &0.559&0.778 &0.668&0.859\\
    P-AUROC & 0.457&0.745 &0.589&0.852\\
    \bottomrule
    \end{tabular}%
    }
   \caption{Performance of the proposed method with different feature extractors.}
  \label{Feature1}
\end{table}


\section{More Parameter Sensitivity Analysis}
\textbf{The influence of parameter $\alpha$.} 
To further examine the effect of the sampling ratio $\alpha=(\alpha_\text{surf}, \alpha_\text{near}, \alpha_\text{uni})$, the proposed method with extremely imbalanced ratios was investigated, and the results are summarized in Table~\ref {NoiseParameter}.

% As shown in Table~\ref {NoiseParameter}, the proposed method with only surface points degraded dramatically, with an 

As shown in Table~\ref {NoiseParameter}, when only surface points are used ($\alpha$ = 2:0:0), the model performance degrades significantly in both O-AUROC and P-AUROC, and the latter is even close to the performance of random guessing. Nevertheless, when increasing the ratio of near-surface points, the AUROC and P-AUROC performance improved by 2.0\% and 4.0\%, respectively. Meanwhile, increasing the ratio of uniform points also enhanced performance, but the improvement was less significant than that achieved by increasing the proportion of near-surface points. The reasons for these results may be that near-surface points provide discriminative feature information, while uniform points offer global spatial distribution information. Both types of information are beneficial for training anomaly detection models. However, excessively introducing uniform points may confuse model learning. Therefore, the sampling ratio is set to $\alpha=(2, 2, 1)$, which well balances the effects of different types of points.

%This result indicates that a single type of surface point cannot provide comprehensive point cloud information support, preventing the model from establishing effective discriminative criteria and thus failing to accurately distinguish target samples.

%Under the conditions of fixing the proportion of surface points ($\alpha_\text{surf} = 2$) while removing uniform points ($\alpha_\text{uni} = 0$), the model performance achieves a leapfrog improvement as the number of near-surface points gradually increases: when the proportion of near-surface points rises from 0 to 1, both O-AUROC and P-AUROC increase sharply. With a further increase in the proportion of near-surface points, O-AUROC continues to rise to its peak, while P-AUROC slightly decreases but remains at a high level. This is because near-surface points have a strong spatial correlation with surface points, which can effectively supplement the fine-grained structural information around the surface and provide the model with key discriminative basis. Their effect on performance improvement is much better than simply increasing the number of surface points. The slight fluctuation of P-AUROC is hypothesized to be due to the gradual weakening of the information utility of near-surface points, which, however, does not affect the overall upward trend.

%Control experiments show that under the conditions of fixing surface points ($\alpha_\text{surf} = 2$) and having no near-surface points ($\alpha_\text{near} = 0$), increasing uniform points can also improve performance, but the effect is significantly inferior to that of adding near-surface points: as the proportion of uniform points gradually increases from 0, both O-AUROC and P-AUROC rise, but the improvement range is limited and always lower than the experimental combination with near-surface points added. Uniform points function to provide global spatial distribution information and mitigate local sampling bias; however, due to their weak correlation with surface features, they cannot accurately supplement key features like near-surface points do, thus restricting the range of performance improvement.

%Experiments and analyses confirm that near-surface points ($P_\text{near}$) and uniform points ($P_\text{uni}$) play indispensable roles in assisting the model to learn discriminative features for 3D anomaly detection.
%Beyond the conventional analysis of parameter $\alpha$, we further investigated the impact of extreme $\alpha$ ratios (i.e., scenarios where the count of one specific type of noise points is set to zero) on model performance. Here, the $\alpha$ ratio denotes the quantity proportion of surface points ($P_\text{surf}$), near-surface noisy points ($P_\text{near}$), and uniform noisy points ($P_\text{uni}$), with the corresponding results summarized in Table~\ref {NoiseParameter}. Specifically, when the $\alpha$ ratio is configured to include only $P_\text{surf}$ and $P_\text{uni}$, or $P_\text{surf}$ and $P_\text{near}$, the model achieves higher performance compared to the scenario where only $P_\text{surf}$ is included. This observation further validates the indispensable role of both $P_\text{near}$ and $P_\text{uni}$ in facilitating the model to learn discriminative features for 3D anomaly detection, which aligns with the findings from the conventional parameter $\alpha$ analysis.

 \begin{table}[htbp]
  \centering
  \resizebox{0.95\columnwidth}{!}{
    \begin{tabular}{c|cccccc}
    \toprule
    \textbf{$\alpha$} & 2:0:0 & 2:1:0 & 2:2:0 & 2:2:1 & 2:0:1 & 2:0:2 \\
    \midrule
    O-AUROC & 0.581&0.804&0.839& 0.859& 0.761& 0.795\\
    P-AUROC & 0.501&0.817&0.812& 0.852& 0.703& 0.757 \\
    \bottomrule
    \end{tabular}%
 }
   \caption{Effect on performance under extremely imbalanced sampling ratios. }
  \label{NoiseParameter}
\end{table}

\section{Result Visualization}
\subsection{Visualizations of Generated Points}
% Fig.~\ref{visNoisy3} visualizes the surface points $P_\text{surf}$, near-surface noisy points $P_\text{near}$, and uniform noisy points $P_\text{uni}$ generated by our Noisy Points Generation (NPG) module. 

%一种类型一种类型的解释，首先说表面点（说明他是用来替换原点云的），然后讲近表面，再说均匀点
Fig.~\ref{visNoisy3} visualizes the surface points $P_\text{surf}$, near-surface noisy points $P_\text{near}$, and uniform noisy points $P_\text{uni}$ generated by our Noisy Points Generation (NPG) module, respectively.
Specifically, the surface points $P_\text{surf}$ are sampled with the probability proportional to the area of the triangular mesh and are relatively uniformly distributed on the surface of the point clouds. The near-surface noisy points $P_\text{near}$ are obtained by adding Gaussian noise to the surface points, and the uniform noisy points are uniformly sampled within the 3D point cloud space.

It can be seen that the near-surface noisy points $P_\text{near}$ (yellow color) adhere closely to the surface of the input point cloud, and this characteristic effectively limits the distribution of normal points and also provides discriminative information for the training of anomaly detection models. Meanwhile, the uniform noisy points $P_\text{uni}$ (gray color) are uniformly sampled within the normalized 3D space $\mathbb{B}=[-1,1]^3$. This sampling method enables noisy points to fill the regions not covered by the near-surface points. The uniform characteristic further enhances the model's ability to detect anomalies in different scales.

%Specifically, $P_\text{surf}$ are  points sampled based on area proportion; $P_\text{near}$ are near-surface noisy points obtained by adding Gaussian noise to the point cloud surface; and $P_\text{uni}$ are uniform noisy points within the point cloud space. It can be observed that $P_\text{near}$ adheres closely to the surface of the input point cloud, and this characteristic effectively mitigates the boundary blurriness issue that may occur during point cloud surface modeling. Meanwhile, $P_\text{uni}$ is uniformly sampled within the normalized 3D space $\mathbb{B}=[-1,1]^3$. This sampling method enables $P_\text{uni}$ to fill the gaps in supervision signals for regions not covered by surface points. The more uniform characteristic of $P_\text{surf}$ compared to the original point cloud, along with the complementary design of $P_\text{near}$ and $P_\text{uni}$, further enhances the model's ability to detect anomalies in different scales.

%Fig.~\ref{visNoisy3} visualizes the surface points $P_\text{surf}$, near-surface noisy points $P_\text{near}$, and uniform noisy points $P_\text{uni}$ generated by our Noisy Points Generation (NPG) module.  Specifically, $P_\text{surf}$ are points sampled based on area proportion; $P_\text{near}$ are near-surface noisy points obtained by adding Gaussian noise to the point cloud surface; and $P_\text{uni}$ are uniform noisy points within the point cloud space. It can be observed that $P_\text{near}$ adheres closely to the surface of the input point cloud, and this characteristic effectively mitigates the boundary blurriness issue that may occur during point cloud surface modeling. Meanwhile, $P_\text{uni}$ is uniformly sampled within the normalized 3D space $\mathbb{B}=[-1,1]^3$. This sampling method enables $P_\text{uni}$ to fill the gaps in supervision signals for regions not covered by surface points. The more uniform characteristic of $P_\text{surf}$ compared to the original point cloud, along with the complementary design of $P_\text{near}$ and $P_\text{uni}$, further enhances the model's ability to detect anomalies in different scales.
%Fig.~\ref{visNoisy3} presents the visualization results of surface points ($P_\text{surf}$), near-surface noisy points ($P_\text{near}$), and uniform noisy points ($P_\text{uni}$). All three types of points are generated by the Noisy Points Generation (NPG) module introduced in Section 3.1. It can be observed that $P_\text{near}$ adheres closely to the surface of the input point cloud, and this characteristic effectively mitigates the boundary blurriness issue that may occur during point cloud surface modeling.

% Meanwhile, $P_\text{uni}$ is uniformly sampled within the normalized 3D space $\mathbb{B}=[-1,1]^3$. This sampling method enables $P_\text{uni}$ to fill the gaps in supervision signals for regions not covered by surface points. The complementary design of $P_\text{near}$ and $P_\text{uni}$ further enhances the model's ability to detect anomalies in different scales.

\begin{figure*}[ht]
  \centering
  % \columnwidth textwidth
    \includegraphics[width=\linewidth]{Supplementary Material/visNoisy4.pdf}
    % \includegraphics[width=\linewidth]{Supplementary Material/visNoisy3.pdf}
  \caption{Visualization of the generated points on the Real3D dataset, with the blue, yellow, and gray points representing the surface points $P_\text{surf}$, near-surface noisy points $P_\text{near}$, and uniform noisy points $P_\text{uni}$, respectively.}
  \label{visNoisy3}
  
\end{figure*}
\begin{figure*}[ht]
  \centering
  % \columnwidth textwidth
  \includegraphics[width=\linewidth]{Supplementary Material/SDF_vis.pdf}
  %\caption{Visualization of 3D shape results of different sampling methods via the SDF model on the Real3D dataset.}
  \caption{Visualization of the distributions and the SDF values of the original and generated point clouds on the Real3D dataset, with higher red color indicating larger SDF values.}
  \label{visSDF}
\end{figure*}

\subsection{Visualizations of Point Distribution and the Learned SDF}
%首先描述现实，用生成的点替换原来的点。然后说为了体现生成点的优势，比较两者的点云和SDF的差异。
%首先分析原点云和生成点云的差异，说明生成点云的优势
% %再分析从两个不同点云上学到的SDF的差异，体现原点云会存在较大误差，并分析原因。
To mitigate the non-uniformity and sparsity of the original input point clouds, surface points are generated using the proposed NPG model. These points, rather than the original points, serve as the normal points for training the discriminative SDF network. To illustrate the advantages of the generated surface points over the original input points, their point distribution and corresponding SDF values are visualized in Figure \ref{visSDF}.

As shown in Figure \ref{visSDF}, the original point clouds (the first row) exhibit local unevenness, and their SDF values (the third row) also have relatively large errors (red points within the white bounding box). In contrast, the generated surface points (the second row) are distributed more uniformly on the surface of the point clouds, and their SDF values (the fourth row) tend toward 0. These results demonstrate the superiority of the generated surface points in learning the surface representation of point clouds using the discriminative SDF networks. 

% To validate the 3D shape reconstruction performance of the trained model and evaluate the proposed area-based surface point sampling method, we conducted experiments on the Real3D dataset using both the original point cloud and the aforementioned surface-sampled generated points. The trained SDF network was employed to fit these two types of point data, and the corresponding visualization results are presented in Figure \ref{visSDF}. As observed from the visualization results, compared with the surface-sampled generated points, the original point cloud exhibits a non-uniform point distribution, and its fitting performance is inferior to that of the former. These results confirm t
%To verify the 3D shape reconstruction performance of the trained model and evaluate $P_\text{surf}$ derived from the proposed area-based surface point sampling method, we replaced the traditional original point cloud with $P_\text{surf}$ in the model training task. The difference between these two types of point clouds lies in their distribution. Limited by acquisition conditions, the original point cloud has an extremely uneven distribution and cannot fully represent the surface topological structure. In contrast, the area-based surface point sampling method performs sampling according to the area proportion, resulting in a much more uniform overall distribution of the generated point cloud. To clearly demonstrate the advantages of the generated points, we designed a comparative experiment on the Real3D dataset, using the original point cloud and the surface-sampled generated points as inputs respectively. The trained Signed Distance Function (SDF) network was employed to fit these two types of point data, and the corresponding visualization results are shown in Figure \ref{visSDF}. It can be seen from the figures that the SDF fitted based on the original point cloud has large errors, while the surface-sampled generated points achieve better fitting results than the original point cloud. Therefore, $P_\text{surf}$ enables the SDF model to better learn the surface information of the point cloud.

\section{Robustness to Noisy Data}
In practical application scenarios, the complexity of the environment and the instability of devices often lead to noise interference in scanned point clouds. To evaluate the robustness of the proposed method to noisy data, experiments were conducted on the Real3D dataset, where Gaussian noise with a standard deviation of 0, 0.001, 0.003, 0.005, or 0.01 was injected into test samples (a standard deviation of 0 indicates noise-free data). The experimental results are in Figure~\ref {Noise standard deviation}.

Notably, as the noise standard deviation increases, the model performance degrades moderately. Moreover, even in its worst-case noise scenario, the proposed method still outperforms other comparative methods that use clean data without injecting noise. These empirical findings highlight the robustness of our approach to noisy data.

\begin{figure}[ht]
  \centering
  % \columnwidth textwidth
  \includegraphics[width=\columnwidth]{AAAI2026_Xiaohaibo/Supplementary Material/Noise.pdf}
  \caption{Robustness of the proposed method to test noise.}
  %\caption{The impact of testing noise with different standard deviations on O-AUROC and P-AUROC.}
  \label{Noise standard deviation}
\end{figure}
  




==> Supplementary_Material/results_Anomoly_O_AUPR.tex <==
\begin{table*}[!hb]
  \centering
% \caption{O-AUROC performance of different methods on Real3D-AD across 40 categories, where best and second-place results are highlighted in red and blue, respectively.}
  \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|cccccccccccccc}
    \toprule
    %\multicolumn{15}{c}{\textbf{O-AUROC}} \\
    %\midrule
    \textbf{Method} & \textbf{ashtray0} & \textbf{bag0} & \textbf{bottle0} & \textbf{bottle1} & \textbf{bottle3} & \textbf{bowl0} & \textbf{bowl1} & \textbf{bowl2} & \textbf{bowl3} & \textbf{bowl4} & \textbf{bowl5} & \textbf{bucket0} & \textbf{bucket1} & \textbf{cap0} \\
    \midrule
\textbf{BTF(Raw) (CVPR23’)} & 0.578 & 0.458 & 0.466 & 0.573 & 0.543 & 0.588 & 0.464 & 0.576 & 0.654 & 0.601 & 0.615 & 0.652 & 0.620 & 0.659 \\
\textbf{BTF(FPFH) (CVPR23’)} & 0.651 & 0.551 & 0.644 & 0.625 & 0.602 & 0.576 & 0.648 & 0.515 & 0.499 & 0.632 & 0.699 & 0.483 & 0.648 & 0.618 \\
\textbf{M3DM (CVPR23’)} & 0.632 & 0.642 & 0.763 & 0.674 & 0.451 & 0.525 & 0.515 & 0.630 & 0.635 & 0.571 & 0.601 & 0.609 & 0.507 & 0.564 \\
\textbf{PatchCore(FPFH) (CVPR22’)} & 0.445 & 0.608 & 0.615 & 0.677 & 0.579 & 0.548 & 0.545 & 0.611 & 0.620 & 0.575 & 0.541 & 0.604 & 0.565 & 0.585  \\
\textbf{PatchCore(PointMAE)  (CVPR22')} & \textcolor{blue}{0.679} & 0.601 & 0.545 & 0.645 & 0.651 & 0.562 & 0.611 & 0.456 & 0.556 & 0.601 & 0.585 & 0.541 & 0.642 & 0.561 \\
\textbf{CPMF (PR24’)} & 0.453 & 0.655 & 0.588 & 0.592 & 0.505 & 0.775 & 0.621 & 0.601 & 0.418 & 0.683 & 0.685 & 0.662 & 0.501 & 0.601  \\
\textbf{Reg3D-AD (NeurIPS23’)} & 0.588 & 0.608 & 0.632 & 0.695 & 0.474 & 0.494 & 0.515 & 0.495 & 0.441 & 0.624 & 0.555 & 0.632 & 0.714 & 0.693  \\
\textbf{IMRNet (CVPR24’)} & 0.612 & 0.665 & 0.558 & 0.702 & 0.648 & 0.481 & 0.504 & 0.681 & 0.614 & 0.630 & 0.652 & 0.578 & 0.732 & 0.711  \\
\textbf{PO3AD (CVPR25')} & \textcolor{red}{0.999} & \textcolor{blue}{0.809} & \textcolor{blue}{0.927} & \textcolor{blue}{0.959} & \textcolor{blue}{0.962} & \textcolor{blue}{0.946} & \textcolor{blue}{0.905} & \textcolor{blue}{0.888} & \textcolor{blue}{0.927} & \textcolor{red}{0.985} & \textcolor{blue}{0.904} & \textcolor{blue}{0.923} & \textcolor{blue}{0.882} & \textcolor{blue}{0.841}\\
\textbf{Ours} & \textcolor{red}{0.999} & \textcolor{red}{0.999} & \textcolor{red}{0.999} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{0.982} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{blue}{0.976} & \textcolor{red}{0.991} & \textcolor{red}{0.981} & \textcolor{red}{0.922} & \textcolor{red}{0.934}\\




% \textbf{Reg2Inv(NIPS25')} & \textcolor{blue}{0.900} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & 0.807 & 0.656 & 0.585 & 0.852 & 0.818 & 0.813 & \textcolor{red}{0.902} & 0.659
% \\

    \midrule
    \multicolumn{1}{c}{} &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \textbf{Method} & \textbf{cap3} & \textbf{cap4} & \textbf{cap5} & \textbf{cup0} & \textbf{cup1} & \textbf{eraser0} & \textbf{headset0} & \textbf{headset1} & \textbf{helmet0} & \textbf{helmet1} & \textbf{helmet2} & \textbf{helmet3} & \textbf{jar0} & \textbf{micro.} \\
    \midrule
\textbf{BTF(Raw) (CVPR23’)} & 0.612 & 0.515 & 0.653 & 0.601 & 0.701 & 0.425 & 0.379 & 0.515 & 0.559 & 0.388 & 0.615 & 0.526 & 0.428 & 0.613  \\
\textbf{BTF(FPFH) (CVPR23’)} & 0.579 & 0.545 & 0.593 & 0.585 & 0.651 & 0.719 & 0.531 & 0.523 & 0.568 & 0.721 & 0.588 & 0.564 & 0.479 & 0.662 \\
\textbf{M3DM (CVPR23’)} & 0.652 & 0.477 & 0.642 & 0.570 & \textcolor{blue}{0.752} & 0.625 & 0.632 & 0.623 & 0.528 & 0.627 & 0.636 & 0.458 & 0.555 & 0.464  \\
\textbf{PatchCore(FPFH) (CVPR22’)} & 0.457 & 0.655 & 0.725 & 0.604 & 0.586 & 0.584 & 0.701 & 0.601 & 0.525 & 0.630 & 0.475 & 0.494 & 0.499 & 0.332 \\
\textbf{PatchCore(PointMAE)  (CVPR22')} & 0.583 & \textcolor{blue}{0.721} & 0.542 & 0.642 & 0.710 & 0.801 & 0.515 & 0.423 & 0.633 & 0.571 & 0.496 & 0.611 & 0.463 & 0.652  \\
\textbf{CPMF (PR24’)} & 0.541 & 0.645 & 0.697 & 0.647 & 0.609 & 0.544 & 0.602 & 0.619 & 0.333 & 0.501 & 0.477 & 0.645 & 0.618 & 0.655  \\
\textbf{Reg3D-AD (NeurIPS23’)} & 0.711 & 0.623 & 0.770 & 0.531 & 0.638 & 0.424 & 0.538 & 0.617 & 0.600 & 0.381 & 0.618 & 0.468 & 0.601 & 0.614 \\
\textbf{IMRNet (CVPR24’)} & 0.702 & 0.658 & 0.502 & 0.455 & 0.627 & 0.599 & 0.701 & 0.656 & 0.697 & 0.615 & 0.602 & 0.575 & 0.760 & 0.552  \\
\textbf{PO3AD (CVPR25')} & \textcolor{red}{0.906} & \textcolor{red}{0.876} & \textcolor{blue}{0.801} & \textcolor{blue}{0.879} & \textcolor{red}{0.870} & \textcolor{blue}{0.995} & \textcolor{blue}{0.765} & \textcolor{blue}{0.914} & \textcolor{blue}{0.864} & \textcolor{blue}{0.961} & \textcolor{red}{0.934} & \textcolor{blue}{0.849} & \textcolor{blue}{0.915} & \textcolor{blue}{0.803}\\
\textbf{Ours} & \textcolor{blue}{0.730} & 0.688 & \textcolor{red}{0.853} & \textcolor{red}{0.999} & 0.523 & \textcolor{red}{0.999} & \textcolor{red}{1.000} & \textcolor{red}{0.999} & \textcolor{red}{0.926} & \textcolor{red}{0.991} & \textcolor{blue}{0.744} & \textcolor{red}{0.970} & \textcolor{red}{0.999} & \textcolor{red}{0.999} \\



% \textbf{Reg2Inv(NIPS25')} & \textcolor{red}{0.863} & 0.681 & \textcolor{blue}{0.902} & 0.733 & \textcolor{red}{0.933} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & 0.843 & \textcolor{blue}{0.817} & \textcolor{blue}{0.986} & \textcolor{red}{0.875} & \textcolor{blue}{0.876} & \textcolor{red}{1.000} & \textcolor{red}{1.000}
% \\
    \midrule
    \multicolumn{1}{c}{} &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \textbf{Method} & \textbf{shelf0} & \textbf{tap0} & \textbf{tap1} & \textbf{vase0} & \textbf{vase1} & \textbf{vase2} & \textbf{vase3} & \textbf{vase4} & \textbf{vase5} & \textbf{vase7} & \textbf{vase8} & \textbf{vase9} & \textbf{Average} \\
    \midrule
\textbf{BTF(Raw) (CVPR23’)} & 0.624 & 0.535 & 0.594 & 0.562 & 0.441 & 0.413 & 0.717 & 0.428 & 0.615 & 0.547 & 0.416 & 0.482 & 0.549    \\
\textbf{BTF(FPFH) (CVPR23’)} & 0.611 & 0.610 & 0.575 & 0.641 & 0.655 & 0.569 & 0.652 & 0.587 & 0.472 & 0.592 & 0.624 & 0.638 & 0.598  \\
\textbf{M3DM (CVPR23’)} & 0.665 & 0.722 & 0.638 & \textcolor{blue}{0.788} & 0.652 & 0.615 & 0.551 & 0.526 & 0.633 & 0.648 & 0.463 & 0.651 & 0.603 \\
\textbf{PatchCore(FPFH) (CVPR22’)} & 0.504 & 0.712 & 0.684 & 0.645 & 0.623 & 0.801 & 0.481 & 0.777 & 0.515 & 0.621 & 0.515 & 0.660 & 0.588   \\
\textbf{PatchCore(PointMAE)  (CVPR22')} & 0.543 & 0.712 & 0.542 & 0.548 & 0.572 & 0.711 & 0.455 & 0.586 & 0.585 & 0.652 & 0.655 & 0.634 & 0.595    \\
\textbf{CPMF (PR24’)} & \textcolor{blue}{0.681} & 0.639 & 0.697 & 0.632 & 0.645 & 0.632 & 0.588 & 0.655 & 0.518 & 0.432 & 0.673 & 0.618 & 0.597  \\
\textbf{Reg3D-AD (NeurIPS23’)} & 0.675 & 0.676 & 0.599 & 0.615 & 0.468 & 0.641 & 0.651 & 0.505 & 0.588 & 0.455 & 0.629 & 0.574 & 0.584   \\
\textbf{IMRNet (CVPR24’)} & 0.625 & 0.401 & \textcolor{blue}{0.796} & 0.573 & 0.725 & 0.655 & 0.708 & 0.528 & 0.654 & 0.601 & 0.639 & 0.462 & 0.621 \\
\textbf{PO3AD (CVPR25')} & 0.680 & \textcolor{blue}{0.856} & 0.709 & 0.753 & \textcolor{blue}{0.789} & \textcolor{blue}{0.963} & \textcolor{blue}{0.902} & \textcolor{blue}{0.824} & \textcolor{blue}{0.879} & \textcolor{blue}{0.971} & \textcolor{blue}{0.833} & \textcolor{blue}{0.904} & \textcolor{blue}{0.881}\\
\textbf{Ours} & \textcolor{red}{0.811} & \textcolor{red}{0.921} & \textcolor{red}{0.951} & \textcolor{red}{0.847} & \textcolor{red}{0.976} & \textcolor{red}{0.999} & \textcolor{red}{0.926} & \textcolor{red}{0.916} & \textcolor{red}{0.999} & \textcolor{red}{0.999} & \textcolor{red}{0.956} & \textcolor{red}{0.934} & \textcolor{red}{0.936}\\



% \textbf{Reg2Inv(NIPS25')} & 0.577 & \textcolor{red}{0.948} & 0.804 & \textcolor{blue}{0.996} & 0.605 & \textcolor{red}{1.000} & \textcolor{blue}{0.845} & 0.818 & \textcolor{red}{1.000} & 0.643 & \textcolor{blue}{0.818} & \textcolor{red}{0.873} & 0.861
% \\

    \bottomrule

    \end{tabular}%
}
    \caption{The O-AUPR ($\uparrow$) performance of different methods on Anomaly-ShapeNet, where the best and second-place results are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.}
  \label{results1}
\end{table*}


==> Supplementary_Material/results_Anomoly_P_AUPR.tex <==
\begin{table*}[!ht]
  \centering
    % \caption{P-AUROC performance of different methods on Anomaly-ShapeNet across 40 categories, where best and second-place results are highlighted in red and blue, respectively.}
  \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|cccccccccccccc}

    
    \midrule
    \textbf{Method} & \textbf{ashtray0} & \textbf{bag0} & \textbf{bottle0} & \textbf{bottle1} & \textbf{bottle3} & \textbf{bowl0} & \textbf{bowl1} & \textbf{bowl2} & \textbf{bowl3} & \textbf{bowl4} & \textbf{bowl5} & \textbf{bucket0} & \textbf{bucket1} & \textbf{cap0} \\
    \midrule
\textbf{Ours} & 0.365&0.678&0.896&0.157&0.050&0.942&0.590&0.211&0.804&0.591&0.670&0.052&0.793&0.885\\


% \textbf{Reg2Inv(NIPS25')} & 0.785 & {0.991} & {0.995} & 0.849 & 0.817 & {0.983} & 0.828 & 0.822 & 0.761 & 0.788 & 0.824 & 0.610 & 0.855 & 0.861\\

    \midrule
    \multicolumn{1}{c}{} &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \textbf{Method} & \textbf{cap3} & \textbf{cap4} & \textbf{cap5} & \textbf{cup0} & \textbf{cup1} & \textbf{eraser0} & \textbf{headset0} & \textbf{headset1} & \textbf{helmet0} & \textbf{helmet1} & \textbf{helmet2} & \textbf{helmet3} & \textbf{jar0} & \textbf{micro.} \\
    \midrule

\textbf{Ours} & 0.044&0.109&0.243&0.827&0.051&0.260&0.546&0.870&0.788&0.603&0.058&0.864&0.901&0.783\\

% \textbf{Reg2Inv(NIPS25')} & {0.945} & 0.864 & {0.970} & 0.798 & 0.881 & {0.980} & {0.946} & {0.970} & {0.925} & 0.906 & {0.891} & 0.956 & {0.982} & {0.992}\\
    \midrule
    \multicolumn{1}{c}{} &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \textbf{Method} & \textbf{shelf0} & \textbf{tap0} & \textbf{tap1} & \textbf{vase0} & \textbf{vase1} & \textbf{vase2} & \textbf{vase3} & \textbf{vase4} & \textbf{vase5} & \textbf{vase7} & \textbf{vase8} & \textbf{vase9} & \textbf{Average}\\
    \midrule
\textbf{Ours} & 0.119&0.819&0.651&0.347&0.592&0.867&0.737&0.169&0.715&0.825&0.785&0.252 &0.537 \\

% \textbf{Reg2Inv(NIPS25')} & 0.632 & {0.918} & 0.869 & {0.980} & 0.705 & {0.997} & 0.844 & {0.927} & 0.879 & 0.863 & {0.934} & {0.971} & 0.882\\
    \bottomrule
    \end{tabular}%
}
      \caption{The P-AUPR ($\uparrow$) performance of ours methods on Anomaly-ShapeNet}
  \label{results2}
\end{table*}

==> Supplementary_Material/results_Real3D_O_AUPR.tex <==
\begin{table*}[!ht]
  \centering
    % \caption{O-AUROC performance of different methods on Real3D-AD across 12 categories, where best and second-place results are highlighted in red and blue, respectively.}
  \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|cccccccccccccc}
    \toprule
    %\multicolumn{14}{c}{\textbf{O-AUROC}}                                                                         &  \\
    %\midrule
    \textbf{Method} & \textbf{Airplane} & \textbf{Car} & \textbf{Candy} & \textbf{Chicken} & \textbf{Diamond} & \textbf{Duck} & \textbf{Fish} & \textbf{Gemstone} & \textbf{Seahorse} & \textbf{Shell} & \textbf{Starfish} & \textbf{Toffees} & \textbf{Average}  \\
    \midrule
\textbf{BTF(Raw) (CVPR23')} & 0.506 & 0.523 & 0.490 & 0.464 & 0.535 & \textcolor{red}{0.760} & 0.633 & 0.598 & 0.793 & \textcolor{blue}{0.751} & \textcolor{blue}{0.579} & 0.700 & 0.611    \\
\textbf{BTF(FPFH) (CVPR23')} & 0.659 & 0.653 & 0.638 & 0.814 & 0.677 & 0.620 & 0.638 & 0.603 & 0.567 & 0.434 & 0.557 & 0.505 & 0.614    \\
\textbf{M3DM((PointBERT) (CVPR23')} & 0.497 & 0.517 & 0.480 & 0.716 & 0.661 & 0.569 & 0.628 & \textcolor{blue}{0.628} & 0.491 & 0.638 & 0.573 & 0.569 & 0.581   \\
\textbf{M3DM(PointMAE) (CVPR23')} & 0.479 & 0.508 & 0.498 & 0.739 & 0.620 & 0.533 & 0.525 & \textcolor{red}{0.663} & 0.518 & 0.616 & 0.573 & 0.593 & 0.572  \\
\textbf{PatchCore(FPFH) (CVPR22')} & \textcolor{red}{0.852} & 0.611 & 0.553 & 0.872 & 0.569 & 0.506 & 0.642 & 0.411 & 0.508 & 0.573 & 0.491 & 0.506 & 0.591    \\
\textbf{PatchCore(FPFH+Raw)  (CVPR22')} & \textcolor{blue}{0.807} & \textcolor{blue}{0.766} & 0.611 & \textcolor{red}{0.885} & 0.767 & 0.560 & 0.844 & 0.411 & 0.763 & 0.553 & 0.473 & 0.559 & 0.667    \\
\textbf{PatchCore(PointMAE)  (CVPR22')} & 0.747 & 0.555 & 0.576 & 0.864 & 0.801 & 0.488 & 0.720 & 0.444 & 0.546 & 0.590 & 0.561 & 0.708 & 0.633   \\
\textbf{Reg3D-AD (NeurIPS23’)} & 0.703 & 0.753 & \textcolor{blue}{0.824} & \textcolor{blue}{0.884} & 0.884 & 0.588 & 0.939 & 0.454 & 0.787 & 0.646 & 0.491 & 0.721 & 0.723    \\
\textbf{Group3AD (MM24')} & 0.757 & 0.706 & \textcolor{red}{0.837} & 0.674 & \textcolor{blue}{0.932} & 0.612 & \textcolor{blue}{0.981} & 0.533 & \textcolor{blue}{0.842} & 0.648 & 0.567 & \textcolor{blue}{0.785} & \textcolor{blue}{0.740}    \\

\textbf{Ours} & 0.599 & \textcolor{red}{0.974} & 0.816 & 0.849 & \textcolor{red}{0.965} & \textcolor{blue}{0.717} & \textcolor{red}{0.982} & 0.617 & \textcolor{red}{0.967} & \textcolor{red}{0.848} & \textcolor{red}{0.620} & \textcolor{red}{0.943} & \textcolor{red}{0.824}
\\


% \textbf{Reg2Inv(NIPS25')} & 0.818 & 0.758 & \textcolor{red}{1.000} & \textcolor{red}{0.944} & \textcolor{red}{1.000} & 0.750 & 0.672 & \textcolor{red}{0.735} & 0.532 & 0.692 & \textcolor{red}{0.841} & 0.626 & 0.780\\

    \bottomrule
    \end{tabular}%
}
    \caption{The O-AUPR ($\uparrow$) performance of different methods on Real3D-AD, where the best and second-place results are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively}
  \label{results3}
\end{table*}




==> Supplementary_Material/results_Real3D_P_AUPR.tex <==
\begin{table*}[!ht]
  \centering
    % \caption{P-AUROC performance of different methods on Real3D-AD across 12 categories, where best and second-place results are highlighted in red and blue, respectively.}
  \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|cccccccccccccc} 
    \midrule
    \textbf{Method} & \textbf{Airplane} & \textbf{Car} & \textbf{Candy} & \textbf{Chicken} & \textbf{Diamond} & \textbf{Duck} & \textbf{Fish} & \textbf{Gemstone} & \textbf{Seahorse} & \textbf{Shell} & \textbf{Starfish} & \textbf{Toffees} & \textbf{Average} \\
    \midrule
\textbf{BTF(Raw) (CVPR23')} & 0.012 & 0.014 & 0.025 & 0.049 & 0.032 & 0.020 & 0.017 & 0.014 & 0.031 & 0.011 & 0.017 & 0.016 & 0.022    \\
\textbf{BTF(FPFH) (CVPR23')} & \textcolor{blue}{0.027} & 0.028 & 0.118 & 0.044 & 0.239 & \textcolor{red}{0.068} & 0.036 & \textcolor{blue}{0.075} & 0.027 & 0.018 & 0.034 & 0.055 & 0.064  \\
\textbf{M3DM((PointBERT) (CVPR23')} & 0.007 & 0.017 & 0.016 & \textcolor{blue}{0.377} & 0.038 & 0.011 & 0.039 & 0.017 & 0.028 & 0.021 & 0.040 & 0.018 & 0.052    \\
\textbf{M3DM(PointMAE) (CVPR23')} & 0.007 & 0.018 & 0.016 & 0.310 & 0.033 & 0.011 & 0.025 & 0.018 & 0.030 & 0.022 & 0.040 & 0.021 & 0.046   \\
\textbf{PatchCore(FPFH) (CVPR22')} & \textcolor{blue}{0.027} & 0.034 & \textcolor{blue}{0.142} & 0.040 & 0.273 & \textcolor{blue}{0.055} & 0.052 & \textcolor{red}{0.093} & 0.031 & 0.031 & 0.037 & 0.040 & 0.071  \\
\textbf{PatchCore(FPFH+Raw)  (CVPR22')} & 0.016 & 0.160 & 0.092 & 0.045 & \textcolor{blue}{0.363} & 0.034 & 0.266 & 0.066 & \textcolor{blue}{0.291} & 0.049 & 0.035 & 0.055 & 0.123    \\
\textbf{PatchCore(PointMAE)  (CVPR22')} & 0.016 & 0.069 & 0.020 & 0.052 & 0.107 & 0.008 & 0.201 & 0.008 & 0.071 & 0.043 & 0.046 & 0.055 & 0.058    \\
\textbf{Reg3D-AD (NeurIPS23’)} & 0.017 & 0.135 & 0.109 & 0.044 & 0.191 & 0.010 & 0.437 & 0.016 & 0.182 & 0.065 & 0.039 & 0.067 & 0.109    \\
\textbf{Group3AD (MM24')} & 0.018 & \textcolor{red}{0.174} & 0.122 & 0.068 & 0.287 & 0.016 & \textcolor{blue}{0.448} & 0.009 & 0.24 & \textcolor{blue}{0.067} & \textcolor{blue}{0.056} & \textcolor{blue}{0.134} & \textcolor{blue}{0.137}  \\

\textbf{Ours} & \textcolor{red}{0.050} & \textcolor{blue}{0.167} & \textcolor{red}{0.485} & \textcolor{red}{0.508} & \textcolor{red}{0.436} & 0.048 & \textcolor{red}{0.577} & 0.039 & \textcolor{red}{0.715} & \textcolor{red}{0.321} & \textcolor{red}{0.127} & \textcolor{red}{0.445} & \textcolor{red}{0.326}
\\




% \textbf{Reg2Inv(NIPS25')} & {0.923} & {0.944} & {0.969} & {0.910} & {0.979} & {0.937} & 0.846 & {0.907} & 0.645 & {0.906} & {0.840} & 0.737 & {0.878}\\

    \bottomrule
    \end{tabular}%
}
    \caption{The P-AUPR ($\uparrow$) performance of different methods on Real3D-AD,where the best and second-place results are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively}
  \label{results11}
\end{table*}

==> sec/4_results2_2.tex <==
\begin{table*}[!ht]
  \centering
    % \caption{P-AUROC performance of different methods on Anomaly-ShapeNet across 40 categories, where best and second-place results are highlighted in red and blue, respectively.}
  \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|ccccccccccccccccccccc}
    \midrule
    \textbf{Method} & \textbf{ashtray0} & \textbf{bag0} & \textbf{bottle0} & \textbf{bottle1} & \textbf{bottle3} & \textbf{bowl0} & \textbf{bowl1} & \textbf{bowl2} & \textbf{bowl3} & \textbf{bowl4} & \textbf{bowl5} & \textbf{bucket0} & \textbf{bucket1} & \textbf{cap0} & \textbf{cap3} & \textbf{cap4} & \textbf{cap5} & \textbf{cup0} & \textbf{cup1} & \textbf{eraser0} & \textbf{headset0} \\
    \midrule
\textbf{BTF(Raw)(CVPR23’)} & 0.512 & 0.430 & 0.551 & 0.491 & 0.720 & 0.524 & 0.464 & 0.426 & 0.685 & 0.563 & 0.517 & 0.617 & 0.686 & 0.524 & 0.687 & 0.469 & 0.373 & 0.632 & 0.561 & 0.637 & 0.578\\
\textbf{BTF(Raw)(CVPR23')            } & 0.512 & 0.430 & 0.551 & 0.491 & 0.720 & 0.524 & 0.464 & 0.426 & 0.685 & 0.563 & 0.517 & 0.617 & 0.686 & 0.524 & 0.687 & 0.469 & 0.373 & 0.632 & 0.561 & 0.637 & 0.578 \\
\textbf{BTF(FPFH)(CVPR23')           } & 0.624 & 0.746 & 0.641 & 0.549 & 0.622 & 0.710 & 0.768 & 0.518 & 0.590 & 0.679 & 0.699 & 0.401 & 0.633 & 0.730 & 0.658 & 0.524 & 0.586 & 0.790 & 0.619 & 0.719 & 0.620 \\
\textbf{M3DM(CVPR23')                } & 0.577 & 0.637 & 0.663 & 0.637 & 0.532 & 0.658 & 0.663 & 0.694 & 0.657 & 0.624 & 0.489 & 0.698 & 0.699 & 0.531 & 0.605 & 0.718 & 0.655 & 0.715 & 0.556 & 0.710 & 0.581 \\
\textbf{PatchCore(FPFH)(CVPR22')     } & 0.597 & 0.574 & 0.654 & 0.687 & 0.512 & 0.524 & 0.531 & 0.625 & 0.327 & 0.720 & 0.358 & 0.459 & 0.571 & 0.472 & 0.653 & 0.595 & 0.795 & 0.655 & 0.596 & 0.810 & 0.583 \\
\textbf{PatchCore(PointMAE)(CVPR22') } & 0.495 & 0.674 & 0.553 & 0.606 & 0.653 & 0.527 & 0.524 & 0.515 & 0.581 & 0.501 & 0.562 & 0.586 & 0.574 & 0.544 & 0.488 & 0.725 & 0.545 & 0.510 & 0.856 & 0.378 & 0.575 \\
\textbf{CPMF(PR24')                  } & 0.615 & 0.655 & 0.521 & 0.571 & 0.435 & 0.745 & 0.488 & 0.635 & 0.641 & 0.683 & 0.684 & 0.486 & 0.601 & 0.601 & 0.551 & 0.553 & 0.551 & 0.497 & 0.509 & 0.689 & 0.699 \\
\textbf{Reg3D-AD(NeurIPS23')         } & 0.698 & 0.715 & 0.886 & 0.696 & 0.525 & 0.775 & 0.615 & 0.593 & 0.654 & 0.800 & 0.691 & 0.619 & 0.752 & 0.632 & 0.718 & 0.815 & 0.467 & 0.685 & 0.698 & 0.755 & 0.580 \\
\textbf{IMRNet(CVPR24')              } & 0.671 & 0.668 & 0.556 & 0.702 & 0.641 & 0.781 & 0.705 & 0.684 & 0.599 & 0.576 & 0.715 & 0.585 & 0.774 & 0.715 & 0.706 & 0.753 & 0.742 & 0.643 & 0.688 & 0.548 & 0.705 \\
\textbf{ISMP(AAAI25')                } & 0.865 & 0.734 & 0.722 & 0.869 & 0.740 & 0.762 & 0.702 & 0.706 & 0.851 & 0.753 & 0.733 & 0.545 & 0.683 & 0.672 & 0.775 & 0.661 & 0.770 & 0.552 & 0.851 & 0.524 & 0.472 \\
\textbf{DU-Net (Ours)                } & 0.612 & 0.628 & 0.749 & 0.822 & 0.641 & 0.769 & 0.735 & 0.617 & 0.574 & 0.812 & 0.744 & 0.738 & 0.754 & 0.701 & 0.763 & 0.783 & 0.844 & 0.727 & 0.654 & 0.569 & 0.718 \\
\textbf{PO3AD(CVPR25')} & \textcolor{red}{0.962} & 0.949 & 0.912 & 0.844 & \textcolor{blue}{0.880} & 0.978 & \textcolor{red}{0.914} & 0.918 & \textcolor{blue}{0.935} & \textcolor{red}{0.967} & \textcolor{blue}{0.941} & 0.755 & \textcolor{blue}{0.899} & \textcolor{blue}{0.957} & \textcolor{blue}{0.948} & \textcolor{red}{0.940} & 0.864 & \textcolor{blue}{0.909} & \textcolor{red}{0.932} & \textcolor{blue}{0.974} & 0.823 \\
\textbf{PASDF(ICCV25')} & \textcolor{blue}{0.948} & 0.861 & 0.958 & \textcolor{red}{0.948} & 0.865 & 0.868 & 0.891 & \textcolor{red}{0.945} & 0.909 & 0.894 & \textcolor{red}{0.956} & \textcolor{red}{0.899} & 0.816 & 0.824 & \textcolor{red}{0.959} & 0.809 & 0.920 & 0.865 & \textcolor{blue}{0.909} & 0.939 & 0.646 \\
\textbf{Reg2Inv(NIPS25')} & 0.785 & \textcolor{red}{0.991} & \textcolor{red}{0.995} & 0.849 & 0.817 & \textcolor{blue}{0.983} & 0.828 & 0.822 & 0.761 & 0.788 & 0.824 & 0.610 & 0.855 & 0.861 & 0.945 & 0.864 & \textcolor{red}{0.970} & 0.798 & 0.881 & \textcolor{red}{0.980} & \textcolor{red}{0.946}\\
\textbf{Ours} & 0.905 & \textcolor{blue}{0.958} & \textcolor{blue}{0.971} & \textcolor{blue}{0.924} & \textcolor{red}{0.891} & \textcolor{red}{0.985} & \textcolor{blue}{0.909} & \textcolor{blue}{0.919} & \textcolor{red}{0.953} & \textcolor{blue}{0.933} & 0.907 & \textcolor{blue}{0.791} & \textcolor{red}{0.939} & \textcolor{red}{0.962} & 0.873 & \textcolor{blue}{0.891} & \textcolor{blue}{0.957} & \textcolor{red}{0.971} & 0.841 & 0.945 & \textcolor{blue}{0.940} \\


    \midrule
    \multicolumn{1}{c}{} &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \textbf{Method} & \textbf{headset1} & \textbf{helmet0} & \textbf{helmet1} & \textbf{helmet2} & \textbf{helmet3} & \textbf{jar0} & \textbf{micro} & \textbf{shelf0} & \textbf{tap0} & \textbf{tap1} & \textbf{vase0} & \textbf{vase1} & \textbf{vase2} & \textbf{vase3} & \textbf{vase4} & \textbf{vase5} & \textbf{vase7} & \textbf{vase8} & \textbf{vase9} & \multicolumn{2}{c}{\textbf{Average}} \\
    \midrule
\textbf{BTF(Raw)(CVPR23')            } & 0.475 & 0.504 & 0.449 & 0.605 & 0.700 & 0.423 & 0.583 & 0.464 & 0.527 & 0.564 & 0.618 & 0.549 & 0.403 & 0.602 & 0.613 & 0.585 & 0.578 & 0.550 & 0.564 & \multicolumn{2}{c}{0.550} \\
\textbf{BTF(FPFH)(CVPR23')           } & 0.591 & 0.575 & 0.749 & 0.643 & 0.724 & 0.427 & 0.675 & 0.619 & 0.568 & 0.596 & 0.642 & 0.619 & 0.646 & 0.699 & 0.710 & 0.429 & 0.540 & 0.662 & 0.568 & \multicolumn{2}{c}{0.628} \\
\textbf{M3DM(CVPR23')                } & 0.585 & 0.599 & 0.427 & 0.623 & 0.655 & 0.541 & 0.358 & 0.554 & 0.654 & 0.712 & 0.608 & 0.602 & 0.737 & 0.658 & 0.655 & 0.642 & 0.517 & 0.551 & 0.663 & \multicolumn{2}{c}{0.616} \\
\textbf{PatchCore(FPFH)(CVPR22')     } & 0.464 & 0.548 & 0.489 & 0.455 & 0.737 & 0.478 & 0.488 & 0.613 & 0.733 & 0.768 & 0.655 & 0.453 & 0.721 & 0.430 & 0.505 & 0.447 & 0.693 & 0.575 & 0.663 & \multicolumn{2}{c}{0.580} \\
\textbf{PatchCore(PointMAE)(CVPR22') } & 0.423 & 0.580 & 0.562 & 0.651 & 0.615 & 0.487 & 0.886 & 0.543 & 0.858 & 0.541 & 0.677 & 0.551 & 0.742 & 0.465 & 0.523 & 0.572 & 0.651 & 0.364 & 0.423 & \multicolumn{2}{c}{0.577} \\
\textbf{CPMF(PR24')                  } & 0.458 & 0.555 & 0.542 & 0.515 & 0.520 & 0.611 & 0.545 & 0.783 & 0.458 & 0.657 & 0.458 & 0.486 & 0.582 & 0.582 & 0.514 & 0.651 & 0.504 & 0.529 & 0.545 & \multicolumn{2}{c}{0.573} \\
\textbf{Reg3D-AD(NeurIPS23')         } & 0.626 & 0.600 & 0.624 & 0.825 & 0.620 & 0.599 & 0.599 & 0.688 & 0.589 & 0.741 & 0.548 & 0.602 & 0.405 & 0.511 & 0.755 & 0.624 & 0.881 & 0.811 & 0.694 & \multicolumn{2}{c}{0.668} \\
\textbf{IMRNet(CVPR24')              } & 0.476 & 0.598 & 0.604 & 0.644 & 0.663 & 0.765 & 0.742 & 0.605 & 0.681 & 0.699 & 0.535 & 0.685 & 0.614 & 0.401 & 0.524 & 0.682 & 0.593 & 0.635 & 0.691 & \multicolumn{2}{c}{0.650} \\
\textbf{ISMP(AAAI25')                } & 0.843 & 0.615 & 0.603 & 0.568 & 0.522 & 0.661 & 0.600 & 0.701 & 0.844 & 0.678 & 0.687 & 0.534 & 0.773 & 0.622 & 0.546 & 0.580 & 0.747 & 0.736 & 0.823 & \multicolumn{2}{c}{0.691} \\
\textbf{DU-Net (Ours)                } & 0.749 & 0.718 & 0.737 & 0.744 & 0.682 & 0.771 & 0.648 & 0.740 & 0.728 & 0.743 & 0.699 & 0.648 & 0.650 & 0.731 & 0.765 & 0.711 & 0.728 & 0.762 & 0.581 & \multicolumn{2}{c}{0.712} \\
\textbf{PO3AD(CVPR25')} & 0.907 & 0.878 & \textcolor{blue}{0.948} & \textcolor{red}{0.932} & 0.846 & 0.871 & 0.810 & 0.663 & 0.783 & 0.692 & \textcolor{blue}{0.955} & \textcolor{blue}{0.882} & \textcolor{blue}{0.978} & \textcolor{blue}{0.884} & \textcolor{blue}{0.902} & \textcolor{red}{0.937} & \textcolor{red}{0.982} & \textcolor{red}{0.950} & 0.952 & \multicolumn{2}{c}{\textcolor{blue}{0.899}} \\
\textbf{PASDF(ICCV25')} & 0.948 & \textcolor{red}{0.944} & \textcolor{red}{0.951} & \textcolor{blue}{0.902} & \textcolor{blue}{0.963} & 0.875 & 0.915 & \textcolor{blue}{0.797} & 0.863 & \textcolor{blue}{0.919} & 0.926 & \textcolor{red}{0.884} & 0.951 & \textcolor{blue}{0.884} & 0.900 & 0.863 & 0.958 & 0.816 & \textcolor{blue}{0.959} & \multicolumn{2}{c}{0.897} \\
\textbf{Reg2Inv(NIPS25')} & \textcolor{blue}{0.970} & \textcolor{blue}{0.925} & 0.906 & 0.891 & 0.956 & \textcolor{red}{0.982} & \textcolor{red}{0.992} & 0.632 & \textcolor{blue}{0.918} & 0.869 & \textcolor{red}{0.980} & 0.705 & \textcolor{red}{0.997} & 0.844 & \textcolor{red}{0.927} & 0.879 & 0.863 & \textcolor{blue}{0.934} & \textcolor{red}{0.971} & \multicolumn{2}{c}{0.882}\\
\textbf{Ours} & \textcolor{red}{0.974} & 0.913 & 0.944 & 0.859 & \textcolor{red}{0.971} & \textcolor{blue}{0.977} & \textcolor{blue}{0.959} & \textcolor{red}{0.852} & \textcolor{red}{0.947} & \textcolor{red}{0.958} & 0.936 & 0.841 & 0.973 & \textcolor{red}{0.912} & 0.890 & \textcolor{blue}{0.931} & \textcolor{blue}{0.962} & 0.930 & 0.869 & \multicolumn{2}{c}{\textcolor{red}{0.924}} \\

    \bottomrule
    \end{tabular}%
}
      \caption{The P-AUROC ($\uparrow$) performance of different methods on Anomaly-ShapeNet,where the best and second best results are highlighted and underlined, respectively}
  \label{results2}
\end{table*}

\begin{table*}[!ht]
  \centering
    % \caption{P-AUROC performance of different methods on Real3D-AD across 12 categories, where best and second-place results are highlighted in red and blue, respectively.}
  \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|cccccccccccccc}
    \midrule
    \textbf{Method} & \textbf{Airplane} & \textbf{Car} & \textbf{Candy} & \textbf{Chicken} & \textbf{Diamond} & \textbf{Duck} & \textbf{Fish} & \textbf{Gemstone} & \textbf{Seahorse} & \textbf{Shell} & \textbf{Starfish} & \textbf{Toffees} & \textbf{Average} \\
    \midrule
\textbf{BTF(Raw) (CVPR23')            } & 0.564 & 0.647 & 0.735 & 0.609 & 0.563 & 0.601 & 0.514 & 0.597 & 0.520 & 0.489 & 0.392 & 0.623 & 0.571 \\
\textbf{BTF(FPFH) (CVPR23')           } & 0.738 & 0.708 & 0.864 & 0.735 & 0.882 & 0.875 & 0.709 & 0.891 & 0.512 & 0.571 & 0.501 & 0.815 & 0.733 \\
\textbf{M3DM (CVPR23')                } & 0.547 & 0.602 & 0.679 & 0.678 & 0.608 & 0.667 & 0.606 & 0.674 & 0.560 & 0.738 & 0.532 & 0.682 & 0.631 \\
\textbf{PatchCore(FPFH) (CVPR22')     } & 0.562 & 0.754 & 0.780 & 0.429 & 0.828 & 0.264 & 0.829 & \textcolor{red}{0.910} & 0.739 & 0.739 & 0.606 & 0.747 & 0.682 \\
\textbf{PatchCore(PointMAE) (CVPR22') } & 0.569 & 0.609 & 0.627 & 0.729 & 0.718 & 0.528 & 0.717 & 0.444 & 0.633 & 0.709 & 0.580 & 0.580 & 0.620 \\
\textbf{Reg3D-AD (NeurIPS23')         } & 0.631 & 0.718 & 0.724 & 0.676 & 0.835 & 0.503 & 0.826 & 0.545 & 0.817 & 0.811 & 0.617 & 0.759 & 0.705 \\
\textbf{R3D-AD (ECCV24')              } & 0.594 & 0.557 & 0.593 & 0.620 & 0.555 & 0.635 & 0.573 & 0.668 & 0.562 & 0.578 & 0.608 & 0.568 & 0.592 \\
\textbf{ISMP (AAAI25')                } & 0.753 & 0.836 & \textcolor{blue}{0.907} & 0.798 & 0.926 & \textcolor{blue}{0.876} & \textcolor{blue}{0.886} & 0.857 & 0.813 & 0.839 & 0.641 & \textcolor{red}{0.895} & 0.836 \\
\textbf{DU-Net(MM25')} & 0.721 & \textcolor{blue}{0.896} & 0.884 & 0.838 & \textcolor{blue}{0.938} & 0.793 & \textcolor{red}{0.910} & 0.848 & 0.801 & 0.872 & 0.799 & 0.861 & 0.847 \\
\textbf{PASDF(ICCV25')} & 0.777 & 0.802 & 0.546 & 0.768 & 0.699 & 0.782 & 0.837 & 0.654 & \textcolor{red}{0.887} & 0.648 & 0.703 & 0.838 & 0.745 \\

\textbf{Reg2Inv(NIPS25')} & \textcolor{red}{0.923} & \textcolor{red}{0.944} & \textcolor{red}{0.969} & \textcolor{red}{0.910} & \textcolor{red}{0.979} & \textcolor{red}{0.937} & 0.846 & \textcolor{blue}{0.907} & 0.645 & \textcolor{red}{0.906} & \textcolor{blue}{0.840} & 0.737 & \textcolor{red}{0.878}\\
\textbf{Ours} & \textcolor{blue}{0.851} & 0.833 & 0.843 & \textcolor{blue}{0.854} & 0.852 & 0.828 & 0.862 & 0.781 & \textcolor{blue}{0.879} & \textcolor{blue}{0.893} & \textcolor{red}{0.891} & \textcolor{blue}{0.862} & \textcolor{blue}{0.852} \\

    \bottomrule
    \end{tabular}%
}
    \caption{The P-AUROC ($\uparrow$) performance of different methods on Real3D-AD, where the best and second best results are highlighted and underlined, respectively}
  \label{results11}
\end{table*}

==> sec/app.tex <==
\clearpage
\section{Appendix}
\subsection{Robustness and Stability Analysis}
To analyze the robustness of our model to real point clouds with noise, we designed experiments on test samples, where Gaussian noise with a standard deviation $\sigma \in \{0, 0.001, 0.003,0.005, 0.01, 0.05\}$ was injected. The experimental results are shown in Table~\ref {robustness}. 
From the O - AUROC and P - AUROC values in Table 6, at small standard deviations (0.001, 0.003, 0.005), both metrics maintain relatively high and close levels, indicating the model can resist low - level Gaussian noise well as minor noise barely damages the point cloud structure and features. At a moderate level like 0.01, slight fluctuations occur, possibly due to “disturbances” that marginally affect feature extraction.  Nevertheless, even under a perturbation of 0.01 the proposed method remains competitive compared to others, which can be attributed to the NPG module used during training and the FDC module’s ability to effectively disentangle normal and abnormal features.

 \begin{table}[t!]
  \centering
  \resizebox{0.95\columnwidth}{!}{
    \begin{tabular}{c|ccccccc}
    \toprule
    \textbf{Deviations} & 0.001 & 0.003 & 0.005 & 0.01& 0.05 \\
    \midrule
    O-AUROC & 0.856&0.854&0.853& 0.857&0.841 \\
    P-AUROC & 0.844&0.841&0.843& 0.840&0.800 \\

    \bottomrule
    \end{tabular}%
 }
   \caption{Detection and localization performance with different levels of noise.}
  \label{robustness}
\end{table}

\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]{fig/vis.pdf}
  \caption{Visualization of anomalies detected in Real3D-AD, where deeper colors indicate a higher probability of being anomalies.}
  \label{vis}
\end{figure}
\subsection{Qualitative Results}
Figure~\ref{vis} illustrates the anomaly localization results of six categories from Real3D-AD. Our method effectively learned to distinguish between normal and abnormal points and accurately identified anomalous regions, demonstrating its effectiveness.

\subsection{Parameter Sensitivity Analysis}
To examine the effects of parameters on performance, controlled experiments were conducted on Real3D. 

\textbf{Parameter effects on the NPG module.}
In the experiment, the number of sampling was fixed at 100000 samples, while the other two anomaly sampling methods used parameter \(s\) for anomaly points. Table \ref{LODParameter} shows \(s\) significantly impacts performance: moderate increases improve results, but excessive \(s\) causes declines. Specifically, performance peaked as \(s\) rose from 10000 to 100000, with O-AUROC and P-AUROC increasing by 4.4\% and 1.8\% respectively; further increases led to performance drops. This confirms reasonable \(s\) boosts anomaly detection. Excessively high \(s\) widens the normal-anomaly point gap, hindering the model's ability to balance features during learning. Thus, \(s=100000\) was chosen for all experiments.


 \begin{table}[t!]
  \centering
  \resizebox{0.95\columnwidth}{!}{
    \begin{tabular}{c|ccccccc}
    \toprule
    \textbf{$s$} & 10000 & 50000 & 100000 & 150000  \\
    \midrule
    O-AUROC & 0.815&0.834&0.859& 0.827\\
    P-AUROC & 0.834&0.847&0.852& 0.821 \\
    \bottomrule
    \end{tabular}%
 }
   \caption{Results of the impact of Number of samples on the NPG module. }
  \label{NoiseParameter}
\end{table}

\textbf{Number of LOD on the LFV module.} Table \ref{LODParameter} shows that increasing the number of LOD parameter $l$ improves performance. Raising $l$ from 1 to 5 enhanced O-AUROC and P-AUROC by 1.4\% and 1.6\%, respectively, confirming that high-detail features capture richer information and aid anomaly detection. Nevertheless, higher $l$ increases model complexity; therefore, the LOD count parameter is set to $l=5$ in all experiments.

 \begin{table}[t!]
  \centering
  \resizebox{0.95\columnwidth}{!}{
    \begin{tabular}{c|ccccccc}
    \toprule
    \textbf{$l$} & 1 & 2 & 3 & 4&5  \\
    \midrule
    O-AUROC & 0.845&0.854&0.853& 0.857 & 0.859\\
    P-AUROC & 0.836&0.841&0.848& 0.851 &0.852\\
    \bottomrule
    \end{tabular}%
 }
   \caption{Results of the impact of the number of LOD on the LFV module. }
  \label{LODParameter}
\end{table}


==> sec/pip.tex <==
\section{Approach}
\begin {figure*}[tt]
\centering
\includegraphics [width=\linewidth]{fig/pip2.pdf}
\caption {The overall framework of our method. The NPG module is first used to generate noisy points from registered point clouds. Then, the LFV module is employed to extract multi-scale features. Finally, the SFD module is utilized to learn discriminative surface functions by leveraging the decoupled normal and abnormal features. In inference, the predicted SDF values are considered point anomaly scores.}

\label {DLF3AD_pipeline}
\end {figure*}

==> sec/results1_2.tex <==
\begin{table*}[!ht]
  \centering
% \caption{O-AUROC performance of different methods on Real3D-AD across 40 categories, where best and second-place results are highlighted in red and blue, respectively.}
  \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|ccccccccccccccccccccc}
    \toprule
    %\multicolumn{15}{c}{\textbf{O-AUROC}} \\
    %\midrule
    \textbf{Method} & \textbf{ashtray0} & \textbf{bag0} & \textbf{bottle0} & \textbf{bottle1} & \textbf{bottle3} & \textbf{bowl0} & \textbf{bowl1} & \textbf{bowl2} & \textbf{bowl3} & \textbf{bowl4} & \textbf{bowl5} & \textbf{bucket0} & \textbf{bucket1} & \textbf{cap0} & \textbf{cap3} & \textbf{cap4} & \textbf{cap5} & \textbf{cup0} & \textbf{cup1} & \textbf{eraser0} & \textbf{headset0}\\
    \midrule
    \textbf{BTF(Raw) (CVPR23’)} & 0.578  & 0.410  & 0.597  & 0.510  & 0.568  & 0.564  & 0.264  & 0.525  & 0.385  & 0.664  & 0.417  & 0.617  & 0.321  & 0.564  & 0.527  & 0.468  & 0.373  & 0.403  & 0.521  & 0.525  & 0.378\\
\textbf{BTF(FPFH) (CVPR23’)} & 0.420 & 0.546 & 0.344 & 0.546 & 0.322 & 0.509 & 0.668 & 0.510 & 0.490 & 0.609 & 0.699 & 0.401 & 0.633 & 0.618 & 0.522 & 0.520 & 0.586 & 0.586 & 0.610 & 0.719 & 0.520  \\
\textbf{M3DM (CVPR23’)} & 0.577 & 0.537 & 0.574 & 0.637 & 0.541 & 0.634 & 0.663 & 0.684 & 0.617 & 0.464 & 0.409 & 0.309 & 0.501 & 0.557 & 0.423 & \textcolor{blue}{0.777} & 0.639 & 0.539 & 0.556 & 0.627 & 0.577\\
\textbf{PatchCore(FPFH) (CVPR22’)} & 0.587 & 0.571 & 0.604 & 0.667 & 0.572 & 0.504 & 0.639 & 0.615 & 0.537 & 0.494 & 0.558 & 0.469 & 0.551 & 0.580 & 0.453 & 0.757 & 0.790 & 0.600 & 0.586 & 0.657 & 0.583\\
\textbf{PatchCore(PointMAE) (CVPR22')} & 0.591 & 0.601 & 0.513 & 0.601 & 0.650 & 0.523 & 0.629 & 0.458 & 0.579 & 0.501 & 0.593 & 0.593 & 0.561 & 0.589 & 0.476 & 0.727 & 0.538 & 0.610 & 0.556 & 0.677 & 0.591\\
\textbf{CPMF (PR24’)} & 0.353 & 0.643 & 0.520 & 0.482 & 0.405 & 0.783 & 0.639 & 0.625 & 0.658 & 0.683 & 0.685 & 0.482 & 0.601 & 0.601 & 0.551 & 0.553 & 0.697 & 0.497 & 0.499 & 0.689 & 0.643\\
\textbf{Reg3D-AD (NeurIPS23’)} & 0.597 & 0.706 & 0.486 & 0.695 & 0.525 & 0.671 & 0.525 & 0.490 & 0.348 & 0.663 & 0.593 & 0.610 & 0.752 & 0.693 & 0.725 & 0.643 & 0.467 & 0.510 & 0.538 & 0.343 & 0.537 \\
\textbf{IMRNet (CVPR24’)} & 0.671 & 0.660 & 0.552 & 0.700 & 0.640 & 0.681 & 0.702 & 0.685 & 0.599 & 0.676 & 0.710 & 0.580 & 0.771 & 0.737 & 0.775 & 0.652 & 0.652 & 0.643 & 0.757 & 0.548 & 0.720\\
\textbf{R3D-AD (ECCV24’)} & 0.833 & 0.720 & 0.733 & 0.737 & 0.781 & 0.819 & 0.778 & 0.741 & 0.767 & 0.744 & 0.656 & 0.683 & 0.756 & 0.822 & 0.730 & 0.681 & 0.670 & 0.776 & 0.757 & 0.890 & 0.738\\
\textbf{PO3AD(CVPR25')} & \textcolor{red}{1.000} & \textcolor{blue}{0.833} & \textcolor{blue}{0.900} & 0.933 & 0.926 & \textcolor{blue}{0.922} & \textcolor{blue}{0.829} & 0.833 & 0.881 & \textcolor{red}{0.981} & 0.849 & 0.853 & 0.787 & \textcolor{blue}{0.877} & 0.859 & \textcolor{red}{0.792} & 0.670 & \textcolor{blue}{0.871} & 0.833 & \textcolor{blue}{0.995} & 0.808\\
\textbf{DU-Net(MM25')} & 0.867 & 0.605 & 0.838 & 0.871 & 0.827 & 0.844 & \textcolor{red}{0.869} & \textcolor{blue}{0.952} & 0.839 & 0.859 & 0.776 & 0.838 & 0.822 & 0.859 & 0.775 & 0.736 & 0.739 & 0.869 & 0.776 & 0.644 & 0.741\\
\textbf{PASDF(ICCV25')} & 0.852 & 0.649 & 0.846 & \textcolor{blue}{0.971} & \textcolor{blue}{0.933} & 0.806 & 0.795 & \textcolor{blue}{0.952} & \textcolor{blue}{0.924} & 0.646 & \textcolor{red}{1.000} & \textcolor{blue}{0.912} & 0.812 & 0.775 & \textcolor{red}{1.000} & 0.765 & 0.853 & 0.713 & \textcolor{blue}{0.912} & \textcolor{red}{1.000} & \textcolor{blue}{0.938}\\
\textbf{Reg2Inv(NIPS25')} & \textcolor{blue}{0.900} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & 0.807 & 0.656 & 0.585 & 0.852 & 0.818 & 0.813 & \textcolor{red}{0.902} & 0.659 & \textcolor{blue}{0.863} & 0.681 & \textcolor{blue}{0.902} & 0.733 & \textcolor{red}{0.933} & \textcolor{red}{1.000} & \textcolor{red}{1.000}\\
\textbf{Ours} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{0.9703} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{blue}{0.967} & \textcolor{blue}{0.989} & \textcolor{red}{0.968} & \textcolor{blue}{0.851} & \textcolor{red}{0.896} & 0.688 & 0.712 & \textcolor{red}{0.919} & \textcolor{red}{1.000} & 0.538 & \textcolor{red}{1.000} & \textcolor{red}{1.000}\\


    \midrule
    \multicolumn{1}{c}{} &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule

    \textbf{Method} & \textbf{headset1} & \textbf{helmet0} & \textbf{helmet1} & \textbf{helmet2} & \textbf{helmet3} & \textbf{jar0} & \textbf{micro.}& \textbf{shelf0} & \textbf{tap0} & \textbf{tap1} & \textbf{vase0} & \textbf{vase1} & \textbf{vase2} & \textbf{vase3} & \textbf{vase4} & \textbf{vase5} & \textbf{vase7} & \textbf{vase8} & \textbf{vase9} & \multicolumn{2}{c}{\textbf{Average}} \\
    \midrule
\textbf{BTF(Raw) (CVPR23')            } & 0.515 & 0.553 & 0.349 & 0.602 & 0.526 & 0.420 & 0.563 & 0.164 & 0.525 & 0.573 & 0.531 & 0.549 & 0.410 & 0.717 & 0.425 & 0.585 & 0.448 & 0.424 & 0.564 & \multicolumn{2}{c}{0.493} \\
\textbf{BTF(FPFH) (CVPR23')           } & 0.490 & 0.571 & 0.719 & 0.542 & 0.444 & 0.424 & 0.671 & 0.609 & 0.560 & 0.546 & 0.342 & 0.219 & 0.546 & 0.699 & 0.510 & 0.409 & 0.518 & 0.668 & 0.268 & \multicolumn{2}{c}{0.528} \\
\textbf{M3DM (CVPR23')                } & 0.617 & 0.526 & 0.427 & 0.623 & 0.374 & 0.441 & 0.357 & 0.564 & 0.754 & 0.739 & 0.423 & 0.427 & 0.737 & 0.439 & 0.476 & 0.317 & 0.657 & 0.663 & 0.663 & \multicolumn{2}{c}{0.552} \\
\textbf{PatchCore(FPFH) (CVPR22')     } & 0.637 & 0.546 & 0.484 & 0.425 & 0.404 & 0.472 & 0.388 & 0.494 & 0.753 & 0.766 & 0.455 & 0.423 & 0.721 & 0.449 & 0.506 & 0.417 & 0.693 & 0.662 & 0.660 & \multicolumn{2}{c}{0.568} \\
\textbf{PatchCore(PointMAE) (CVPR22') } & 0.627 & 0.556 & 0.552 & 0.447 & 0.424 & 0.483 & 0.488 & 0.523 & 0.458 & 0.538 & 0.447 & 0.552 & 0.741 & 0.460 & 0.516 & 0.579 & 0.650 & 0.663 & 0.629 & \multicolumn{2}{c}{0.562} \\
\textbf{CPMF (PR24')                  } & 0.458 & 0.555 & 0.589 & 0.462 & 0.520 & 0.610 & 0.509 & 0.685 & 0.359 & 0.697 & 0.451 & 0.345 & 0.582 & 0.582 & 0.514 & 0.618 & 0.397 & 0.529 & 0.609 & \multicolumn{2}{c}{0.559} \\
\textbf{Reg3D-AD (NeurIPS23')         } & 0.610 & 0.600 & 0.381 & 0.614 & 0.367 & 0.592 & 0.414 & 0.688 & 0.676 & 0.641 & 0.533 & 0.702 & 0.605 & 0.650 & 0.500 & 0.520 & 0.462 & 0.620 & 0.594 & \multicolumn{2}{c}{0.572} \\
\textbf{IMRNet (CVPR24')              } & 0.676 & 0.597 & 0.600 & 0.641 & 0.573 & 0.780 & 0.755 & 0.603 & 0.676 & 0.696 & 0.533 & 0.757 & 0.614 & 0.700 & 0.524 & 0.676 & 0.635 & 0.630 & 0.594 & \multicolumn{2}{c}{0.661} \\
\textbf{R3D-AD (ECCV24')              } & 0.795 & 0.757 & 0.720 & 0.633 & 0.707 & 0.838 & 0.762 & 0.696 & 0.736 & 0.900 & 0.788 & 0.729 & 0.752 & 0.742 & 0.630 & 0.757 & 0.771 & 0.721 & 0.718 & \multicolumn{2}{c}{0.749} \\
\textbf{PO3AD(CVPR25')} & 0.923 & 0.762 & 0.961 & \textcolor{blue}{0.869} & 0.754 & 0.866 & 0.776 & 0.573 & 0.745 & 0.681 & 0.858 & 0.742 & \textcolor{blue}{0.952} & 0.821 & 0.675 & \textcolor{blue}{0.852} & 0.966 & 0.739 & 0.830 & \multicolumn{2}{c}{0.839} \\
\textbf{DU-Net(MM25')} & \textcolor{blue}{0.961} & 0.743 & 0.860 & 0.841 & 0.859 & 0.744 & \textcolor{blue}{0.837} & 0.688 & 0.739 & 0.840 & 0.833 & 0.808 & 0.644 & 0.766 & 0.749 & 0.838 & 0.844 & 0.808 & 0.525 & \multicolumn{2}{c}{0.797} \\
\textbf{PASDF(ICCV25')} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & 0.793 & \textcolor{red}{1.000} & \textcolor{blue}{0.968} & \textcolor{red}{1.000} & \textcolor{blue}{0.929} & \textcolor{blue}{0.836} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & 0.882 & \textcolor{red}{1.000} & \textcolor{blue}{0.857} & \textcolor{blue}{0.948} & \textcolor{red}{1.000} & \textcolor{blue}{0.995} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \multicolumn{2}{c}{\textcolor{blue}{0.900}} \\
\textbf{Reg2Inv(NIPS25')} & 0.843 & \textcolor{blue}{0.986} & 0.875 & \textcolor{red}{0.876} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & 0.577 & \textcolor{red}{0.948} & 0.804 & \textcolor{blue}{0.996} & 0.605 & \textcolor{red}{1.000} & 0.845 & 0.818 & \textcolor{red}{1.000} & 0.643 & 0.863 & 0.818 & \textcolor{blue}{0.873} & \multicolumn{2}{c}{0.861}\\
\textbf{Ours} & \textcolor{red}{1.000} & 0.849 & \textcolor{blue}{0.990} & 0.713 & \textcolor{blue}{0.945} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & 0.690 & \textcolor{red}{0.848} & 0.930 & \textcolor{blue}{0.933} & \textcolor{blue}{0.967} & \textcolor{red}{1.000} & \textcolor{red}{0.861} & 0.824 & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{blue}{0.924} & \textcolor{blue}{0.873} & \multicolumn{2}{c}{\textcolor{red}{0.921}} \\
    \bottomrule
    
    \end{tabular}%
}
    \caption{The O-AUROC ($\uparrow$) performance of different methods on Anomaly-ShapeNet, where the best and second-best results are highlighted and underlined, respectively.}
  \label{results1}
\end{table*}

\begin{table*}[!ht]
  \centering
    % \caption{O-AUROC performance of different methods on Real3D-AD across 12 categories, where best and second-place results are highlighted in red and blue, respectively.}
  \resizebox{0.95\textwidth}{!}{
    \begin{tabular}{c|ccccccccccccc}
    \toprule
    %\multicolumn{14}{c}{\textbf{O-AUROC}}                                                                         &  \\
    %\midrule
    \textbf{Method} & \textbf{Airplane} & \textbf{Car} & \textbf{Candy} & \textbf{Chicken} & \textbf{Diamond} & \textbf{Duck} & \textbf{Fish} & \textbf{Gemstone} & \textbf{Seahorse} & \textbf{Shell} & \textbf{Starfish} & \textbf{Toffees} & \textbf{Average}  \\
    \midrule
\textbf{BTF(Raw) (CVPR23')} & 0.730 & 0.647 & 0.539 & 0.789 & 0.707 & 0.691 & 0.602 & 0.686 & 0.596 & 0.396 & 0.530 & 0.703 & 0.635 \\
\textbf{BTF(FPFH) (CVPR23')} & 0.520 & 0.560 & 0.630 & 0.432 & 0.545 & 0.784 & 0.549 & 0.648 & 0.779 & 0.754 & 0.575 & 0.462 & 0.603 \\
\textbf{M3DM (CVPR23')} & 0.434 & 0.541 & 0.552 & 0.683 & 0.602 & 0.433 & 0.540 & 0.644 & 0.495 & 0.694 & 0.551 & 0.450 & 0.552 \\
\textbf{PatchCore(FPFH) (CVPR22')} & \textcolor{red}{0.882} & 0.590 & 0.541 & 0.837 & 0.574 & 0.546 & 0.675 & 0.370 & 0.505 & 0.589 & 0.441 & 0.565 & 0.593 \\
\textbf{PatchCore(PointMAE) (CVPR22')} & 0.726 & 0.498 & 0.663 & 0.827 & 0.783 & 0.489 & 0.630 & 0.374 & 0.539 & 0.501 & 0.519 & 0.585 & 0.594 \\
\textbf{CPMF (PR24')} & 0.701 & 0.551 & 0.552 & 0.504 & 0.523 & 0.582 & 0.558 & 0.589 & 0.729 & 0.653 & 0.700 & 0.390 & 0.586 \\
\textbf{Reg3D-AD (NeurIPS23')} & 0.716 & 0.697 & 0.685 & 0.852 & 0.900 & 0.584 & 0.915 & 0.417 & 0.762 & 0.583 & 0.506 & 0.827 & 0.704 \\
\textbf{IMRNet (CVPR24')} & 0.762 & 0.711 & 0.755 & 0.780 & 0.905 & 0.517 & 0.880 & 0.674 & 0.604 & 0.665 & 0.674 & 0.774 & 0.725 \\
\textbf{R3D-AD (ECCV24')} & 0.772 & 0.696 & 0.713 & 0.714 & 0.685 & \textcolor{red}{0.909} & 0.692 & 0.665 & 0.720 & 0.840 & 0.701 & 0.703 & 0.734 \\
\textbf{ISMP (AAAI25')} & \textcolor{blue}{0.858} & 0.731 & 0.852 & 0.714 & 0.948 & 0.712 & 0.945 & 0.468 & 0.729 & 0.623 & 0.660 & 0.842 & 0.767 \\
\textbf{PO3AD(CVPR25')} & 0.804 & 0.654 & 0.785 & 0.686 & 0.801 & 0.820 & 0.859 & 0.693 & 0.756 & 0.800 & \textcolor{blue}{0.758} & 0.771 & 0.766 \\
\textbf{DU-Net(MM25')} & 0.718 & 0.738 & 0.856 & 0.696 & 0.824 & \textcolor{blue}{0.844} & 0.908 & \textcolor{blue}{0.733} & 0.814 & 0.822 & 0.755 & 0.834 & 0.795 \\
\textbf{PASDF(ICCV25')} & 0.628 & \textcolor{red}{0.959} & 0.788 & 0.739 & 0.894 & 0.658 & \textcolor{red}{0.989} & 0.634 & \textcolor{red}{1.000} & \textcolor{blue}{0.850} & 0.617 & \textcolor{blue}{0.866} & \textcolor{blue}{0.802} \\
\textbf{Reg2Inv(NIPS25')} & 0.818 & 0.758 & \textcolor{red}{1.000} & \textcolor{red}{0.944} & \textcolor{red}{1.000} & 0.750 & 0.672 & \textcolor{red}{0.735} & 0.532 & 0.692 & \textcolor{red}{0.841} & 0.626 & 0.780\\
\textbf{Ours} & 0.674 & \textcolor{blue}{0.872} & \textcolor{blue}{0.976} & \textcolor{blue}{0.856} & \textcolor{blue}{0.958} & 0.797 & \textcolor{blue}{0.979} & 0.676 & \textcolor{blue}{0.964} & \textcolor{red}{0.922} & 0.710 & \textcolor{red}{0.920} & \textcolor{red}{0.859} \\

    \bottomrule
    \end{tabular}%
}
    \caption{The O-AUROC ($\uparrow$) performance of different methods on Real3D-AD, where the best and second-best results are highlighted and underlined, respectively.}
  \label{results3}
\end{table*}



